Content Moderation and the Formation of Online Communities: A Theoretical Framework

We study the impact of content moderation policies in online communities. In our theoretical model, a platform chooses a content moderation policy and individuals choose whether or not to participate in the community according to the fraction of user content that aligns with their preferences. The effects of content moderation, at first blush, might seem obvious: it restricts speech on a platform. However, when user participation decisions are taken into account, its effects can be more subtle $\unicode{x2013}$ and counter-intuitive. For example, our model can straightforwardly demonstrate how moderation policies may increase participation and diversify content available on the platform. In our analysis, we explore a rich set of interconnected phenomena related to content moderation in online communities. We first characterize the effectiveness of a natural class of moderation policies for creating and sustaining stable communities. Building on this, we explore how resource-limited or ideological platforms might set policies, how communities are affected by differing levels of personalization, and competition between platforms. Our model provides a vocabulary and mathematically tractable framework for analyzing platform decisions about content moderation.

==> 3_adversary/proofof_adversary.tex <==
\proofofqed{\cref{thm:one_robust}}{
    %
    Without loss of generality, we will just consider the case when switching-from-left stabilizes to size less than $n/2$. (If there is no large exodus from right or left, the platform will do nothing; if there is a large exodus from the left, the argument is symmetric.)
%
    \newcommand{\thetaeff}{\theta^{\text{eff}}}
 %       
    We will first prove that switching-from-left stabilizes to a set of remaining users $\{j, j+1, \dots, n\}$ for some $j \in [n]$. (I.e., there are no ``holes'' after switching stabilizes.) 
    %
    For any nonempty set of users $\cS$, define user $i$'s \textit{effective tolerance} with respect to $\cS$ as
    \begin{align*}
        \thetaeff_i(\cS) \defeq \frac{\abs{\curly{j \in \cS \setminus \{i\} \; \middle| \; {p_j \in [l_i, r_i]}}}}{\abs{\cS}}
    \end{align*}
    to be the proportion of users that are compatible with user $j$.

    At a given step, let $\cW$ be the set of users remaining on the platform.
    %
    We claim that at any point in the switching, for all $i$ such that $\thetaeff_i(\cW) < \theta$, it holds $\thetaeff_i(\cW)$ is non-decreasing in $i$.
    %
    We prove this by showing that departures occur right-to-left except possibly in the case where users find the same set of users compatible, in which case all those users will eventually exit the platform.
    %
    We prove this by induction on user indices. 
    %
    Suppose all users $1, \dots, i-1$ left the platform.
    %
    Then if user $i$ has effective tolerance less than $\theta$, user $i-1$ must have been compatible with them, or else they would still have the same compatibilities as before switching started.
    %
    But since $r_i \leq r_j$ for all $i < j$, there is no other user with fewer compatibilities than user $i$.
    %
    Additionally, any other user who has effective tolerance less than $\theta$ must have been compatible with user $i-1$ or else they would still have the same compatibilities as before switching started.
    %
    If user $j$ has a higher effective tolerance than user $i$, user $i$ is first in the switching order.
    %
    If user $j$ has the same effective tolerance that user $i$ has, we break ties arbitrarily, so user $j$ may depart the platform instead of user $i$.
    %
    But since $j$ had the same effective tolerance, user $j$ and $i$ must have had intervals that covered the same speech points, which means they must have been mutually compatible.
    %
    Thus, user $i$ lost a compatibility when user $j$ left, and since 
    \begin{align*}
        \frac{x}{y} \geq \frac{x-1}{y-1}
    \end{align*}
    for $x, y \in \Z, y \geq 2$, this implies that user $i$ still have effective tolerance less than $\theta$. (Since we can set $x$ to user $i$'s compatibilities before user $j$ exited and $y$ to the number of users before $j$ exited and have the right-hand side represent user $i$'s effective tolerance after $j$ departs.)
    %
    Since we just proved only users who are mutually compatible with user $i$ can exit the platform before user $i$ does, user $i$ must eventually leave the platform.
    %
    This implies that if the platform is stable and user $i$ is off the platform, so must be user $i-1$.
        
    
    Let $q$ be the index of the last user that leaves after switching-from-left,
    %
    %
    and let
    \begin{align*}
        u \defeq \min\curly{q, n-\ceil{(1-\theta)/\theta}}.
    \end{align*}
    %
    For our window, we will choose the interval $[p_1, p_u]$.
    %
    Now we will argue that if any one user from the set $\{1, \dots, u\}$ is removed, the rest will stay and the platform is stable.

    Suppose user $i$ is removed. Now consider user $j$'s compatibilities.
    %
    If user $u$ is not compatible with user $j$, we know that user $j$ will not have effective tolerance less than $\theta$ because at least $\ceil{(1-\theta)/\theta}$ users were eliminated from the original set and since user $j$ is not compatible with user $u$, they were also not compatible with any of the $\ceil{(1-\theta)/\theta}$ users at the right-end of the interval that were removed.
    %
    Now suppose user $u$ is compatible with user $j$. 
    %
    Then user $j$ is compatible with every user to their right and since 
    \begin{align*}
        \frac{L_j}{j-1} \geq \theta,
    \end{align*}
    this implies that user $j$'s effective tolerance is greater than $\theta$.
}



==> relatedwork.tex <==
\paragraph{Schelling's Bounded Neighborhood Model and threshold models.} Our model builds on an exploration of tipping, initiated by \citet{schelling1971dynamic}, which considers how mild in-group preferences of individuals within communities can lead to large disparities in their demographic composition.
%
Our work generalizes the Bounded Neighborhood Model proposed in Schelling's work by allowing for more heterogeneity among individuals: in the original model, individuals come from two types and have preferences for members of their own group; the focus in his model is on a single neighborhood, which corresponds to the single platform model analyzed in \cref{sec:model} through \cref{sec:adversaries}. Individuals in Schelling's model come from one of two demographic groups: this can be represented in our model by placing individuals in two stacks, one for each demographic group; individuals of a given type have intervals that cover their stack but disjoint from the other. 
%
In Schelling's model, individuals of each group have a continuum of participation thresholds, and, within a group, individuals with the most utility to gain by moving into or out of the neighborhood (or platform, in our context) get to move first; by contrast, our results hold for any choice of switching order.

A general and closely related class of models originated by \citet{granovetter1978threshold} were used to describe the spread of information, decisions to participate in public protests and the adoption of new technologies.
%
In these models, individuals can be in one of two states, either adopting or unadopting: in our context, users are either \textit{on} or \textit{off} the platform.
%
In the canonical threshold model, each individual will adopt a new innovation or behavior if a high enough proportion of the population has already done so.
%
Our model is distinguished from these models by the fact that individuals may also \textit{discourage} adoption (i.e., participation in the platform) by producing content that the individuals dislike, in addition to encouraging it by producing content they like. This introduces meaningful heterogeneity in relationships between individuals in the community, and allows us to answer different questions: e.g., how should some users should be excluded from adoption in order for others to be willing to adopt?

Recently, other threshold models have been used to analyze how platforms would choose moderation policies based on their revenue sources.
%
\citet{liu2022implications} compares advertising- versus subscription-based revenue models for social media companies and computes the equilibrium profit-maximizing content moderation policies for each revenue model.
%
Their model of user content consumption and creation on an axis is similar to a special case of ours: every user is willing to consume content that is less extreme than their speech and dislikes content that is more extreme than theirs; in our model, this corresponds to the case where, e.g., the left interval endpoints $l_i$ of each user $i$ are all the same and user speech points $p_i$ are equal to their right endpoints $r_i$.
%
%This special case allows for analytical solutions to the size of the equilibrium induced by content moderation.

\citet{madio2023content} also consider the effect of content moderation on revenue, endogenizing advertisers' decisions and assuming all users have identical preferences over the content space.%; they consider a model where advertisers derive negative utility from ``unsafe'' content but users may either derive utility or disutility from it.
%
They derive equilibrium prices of advertisements under the assumption that advertisers may suffer reputational damages as a result of harmful content on the platform, whereas users may either all derive utility from the harmful content or all derive disutility from it.
%
Our user model allows for significantly more heterogeneity in users (e.g., user preferences can be any interval, speech point combination), considers switching dynamics (rather than assuming the user base is the largest Nash equilibrium), and makes no distributional assumptions about the arrangement of user preferences in the population.
%
These yield a richer set of possible questions to ask and outcomes to explore: for example, we can explore how the delicate relationships between user preferences may trigger cascades in our model and thus compare the power of window-based moderation to a theoretical optimum; by contrast, their equilibria are the solution to a fixed point in a pair of equations over users' utilities and revenue over a uniform distribution of user preferences.
%
Additionally, we do not make assumptions about the possible revenue models of platforms, instead opting to examine the more basic question of how moderation would affect the size of the platform.
%

%\mr{Is there any follow-up work on Schelling worth mentioning here?}
%

%
%For example, the SI(S) model (susceptible/infected/(susceptible)) describes the transmission of disease through society \cite{hethcote1989three}, where the optional last state specifies whether individuals can recover and be reinfected, and analyzes the size of the infected population over time.
%
%In the model, each infected individual transmits the disease to a susceptible social contact with some probability and, if it is the SIS model, recovers with some probability.
% 

\paragraph{Opinion dynamics models.}
Significant effort has been dedicated to understanding how individuals change over time as a result of their interactions with the social contacts \cite{acemoglu2011opinion}.
%
In the canonical voter model \cite{clifford1973model}, each individual would determine the probability they join the platform by the (weighted) majority vote of their social contacts.
%
Others, such as \citet{degroot1974reaching}'s famous model, extend this setup to settings where opinions are continuous rather than binary, and subsequent research extended these models to sophisticated, rational Bayesian agents \cite{PARIKH1990178}.

Opinion dynamics models have recently been used in an analysis of the effects of platforms choosing moderation policies to affect the spread of harmful ideas or misinformation.
%
\citet{mostagir2022naive} compare the effectiveness of various content moderation policies on the spread of misinformation in a model of agents under DeGroot and Bayesian learning. 
%
The same authors in a different paper analyze the relative effectiveness of quarantining or banning online communities under a simple behavioral model of how individuals join communities and change their views over time \cite{mostagir2023should}. 
%
Our focus is on how moderation policies affect members' willingness to participate and the interactions between user preferences and platform choices that result.
%
Thus, our model is appropriate to contexts where the platform is choosing policies strategically based on the overall impact it will have on the size of the community rather than the impact it will have on the spread of misinformation. 
%
Additionally, individuals do not change their minds in our model, allowing us to study how macro-scale phenomena can emerge from the interactions of micro-scale individual behavior, even if individuals themselves do not change. We consider a generalization of the model with dynamic speech and preferences in \cref{sec:modelextensions}.

%Their results consider how spill-over effects from new membership behavior (and changes to members' beliefs) resulting from these platform actions over the short and long term.
%
%The analysis in \citet{mostagir2023should} considers platform interventions at the scale of communities (i.e., whether to ban communities or make it harder for users to find and engage with them) whereas our analysis focuses on decisions to moderate allowable content itself. 
%
%In contexts like subreddits and Facebook groups considered in \citet{mostagir2023should}, our model complements theirs by considering moderators' decisions to choose what content is allowed \textit{within} a community. 
%
%Our model also captures a broad range of platforms where there is personalization or where different platforms are competing for users (rather than the same platform hosting multiple different groups).
%

\paragraph{Network cascade and unravelling models.} Other models center on user choices to participate in social networks, where individuals are represented by nodes in a graph and two nodes form an edge if the individuals know each other.
%
\citet{bhawalkar2015preventing} consider the problem of how to prevent a network from unravelling if each node must have a certain number of edges to stay; i.e., how to find large $k$-cores if the platform can artificially exempt some nodes from the minimum degree requirement.
%
In their model, the platform can choose a small number of users that will stay on the platform, and they prove inapproximability results for finding the largest equilibrium size of the community.
%
Similarly, \citet{chesney2015critical} simulate a similar model, and find that in some circumstances, a very small number of departures in the networks can cause it to unravel.
%
In our model, unlike these ones, personal relationships between users is not the main reason that users participate; instead, users participate because of the content available in a community, rather than the presence of their social contacts.


\paragraph{Other microfounded models.} Other microfounded analyses explore the interplay between individual preferences and information-mediating institutions, such as how polarization can emerge even if everyone receives the same signal about the world from a public official \cite{glaeser2014does}, how fake news can spread farther than real news even when agents agree on the credibility of any given piece of news \cite{hsu2021persuasion} and how news subscribers may rationally prefer biased news sources \cite{suen-biased-beliefs, hsu2021information}. 
%
To the best of our knowledge, our model is the first to provide a framework for analyzing interactions between moderation policies and user preferences.

%\mr{Relevant: \url{https://siderius.lids.mit.edu/wp-content/uploads/sites/36/2023/01/quarantine-v6.pdf}. Should also check references here}

%\mr{Generally should add more related work}
